Tame Circle Actions

In this paper, we consider Sjamaar's holomorphic slice theorem, the birational equivalence theorem of Guillemin and Sternberg, and a number of important standard constructions that work for Hamiltonian circle actions in both the symplectic category and the K\"ahler category: reduction, cutting, and blow-up. In each case, we show that the theory extends to Hamiltonian circle actions on complex manifolds with tamed symplectic forms. (At least, the theory extends if the fixed points are isolated.) Our main motivation for this paper is that the first author needs the machinery that we develop here to construct a non-Hamiltonian symplectic circle action on a closed, connected six-dimensional symplectic manifold with exactly 32 fixed points; this answers an open question in symplectic geometry. However, we also believe that the setting we work in is intrinsically interesting, and elucidates the key role played by the following fact: the moment image of $e^t \cdot x$ increases as $t \in \mathbb{R}$ increases.

==> metamatter.tex <==
%Note that this file uses the ifthen and hyperref LaTeX packages.

%Diagram options

\input xy
\xyoption{all}

%Space between paragraphs:

\setlength{\parskip}{.5\baselineskip}

% "End of Example" symbol - thanks to Yael Karshon for this:
\def\eoe{\unskip\ \hglue0mm\hfill$\between$\smallskip\goodbreak}

% -- To Make Parenthetical Titles Bold

\makeatletter
\def\th@plain{%
  \thm@notefont{}% same as heading font
  \itshape % body font
}
\def\th@definition{%
  \thm@notefont{}% same as heading font
  \normalfont % body font
}
\makeatother


%Notations - \mathbb

\renewcommand{\AA}{{\mathbb{A}}} %adeles or affine
\newcommand{\BB}{{\mathbb{B}}}  %unit ball
\newcommand{\CC}{{\mathbb{C}}}  %complex numbers
\newcommand{\DD}{{\mathbb{D}}}  %unit disk
\newcommand{\EE}{{\mathbb{E}}}  %euclidean space
\newcommand{\FF}{{\mathbb{F}}}  %field
\newcommand{\HH}{{\mathbb{H}}}  %quaternion numbers
\newcommand{\NN}{{\mathbb{N}}}  %natural numbers
\newcommand{\PP}{{\mathbb{P}}}  %projective
\newcommand{\QQ}{{\mathbb{Q}}}  %rational numbers
\newcommand{\RR}{{\mathbb{R}}}  %real numbers or cartesian space
\renewcommand{\SS}{{\mathbb{S}}} %sphere
\newcommand{\TT}{{\mathbb{T}}}  %torus
\newcommand{\XX}{{\mathbb{X}}}  %dunno...
\newcommand{\ZZ}{{\mathbb{Z}}}  %integers

%Notations - \operatorname

\newcommand{\Ad}{{\operatorname{Ad}}}  %adjoint operator
\newcommand{\ad}{{\operatorname{ad}}}  %infinitesimal adjoint operator
\newcommand{\Alt}{{\operatorname{Alt}}}  %alternating functor
\newcommand{\Aut}{{\operatorname{Aut}}}  %automorphisms
\newcommand{\curv}{{\operatorname{curv}}}   %curvature
\newcommand{\D}{{\operatorname{D}}}  %differential operator
\newcommand{\Der}{{\operatorname{Der}}}  %derivations functor
\newcommand{\Diff}{{\operatorname{Diff}}}  %diffeomorphisms
\newcommand{\End}{{\operatorname{End}}}  %endomorphisms
\newcommand{\ev}{{\operatorname{ev}}}   %evaluation map
\renewcommand{\Gauge}{{\operatorname{Gauge}}} %Gauge groupoid
\newcommand{\Gr}{{\operatorname{Gr}}}  %Gromov-Witten invariant
\newcommand{\Grc}{{\operatorname{Gr}_0}} %connected Gromov-Witten invariant
\newcommand{\Ham}{{\operatorname{Ham}}} %hamiltonian diffeomorphisms
\newcommand{\ham}{{\operatorname{ham}}} %hamiltonian vector fields
\newcommand{\Hol}{{\operatorname{Hol}}} %holonomy group
\newcommand{\Hom}{{\operatorname{Hom}}} %Hom
\newcommand{\id}{{\operatorname{id}}}  %identity
\newcommand{\im}{{\operatorname{im}}}  %image
\newcommand{\inter}{{\operatorname{int}}} %interior
\newcommand{\Mat}{{\operatorname{Mat}}} %matrices
\newcommand{\PD}{{\operatorname{PD}}}  %Poincare dual
\newcommand{\pr}{{\operatorname{pr}}} %projection
\newcommand{\Rep}{{\operatorname{Rep}}} %representations
\newcommand{\rk}{{\operatorname{rk}}}  %rank
\newcommand{\sgn}{{\operatorname{sgn}}}  %signum
\newcommand{\Span}{{\operatorname{span}}}  %span
\newcommand{\Stab}{{\operatorname{Stab}}} %stabiliser
\newcommand{\supp}{{\operatorname{supp}}}  %support
\newcommand{\Sym}{{\operatorname{Sym}}}  %symmetric functor
\newcommand{\Symp}{{\operatorname{Symp}}} %symplectomorphisms
\newcommand{\Vect}{{\operatorname{vect}}}  %vector fields

%Notations - Lie

\newcommand{\G}{{\operatorname{G}}} %generic Lie group
\newcommand{\g}{{\mathfrak{g}}} %generic Lie algebra
\newcommand{\GL}{{\operatorname{GL}}}  %general linear
\newcommand{\lie}[1]{{\mathfrak{\lowercase{#1}}}} %Lie algebra of a Lie group
\renewcommand{\O}{{\operatorname{O}}} %orthogonal
\newcommand{\SL}{{\operatorname{SL}}}  %special linear
\newcommand{\SO}{{\operatorname{SO}}}  %special orthogonal
\newcommand{\Sp}{{\operatorname{Sp}}} %symplectic linear
\newcommand{\SU}{{\operatorname{SU}}}  %special unitary
\newcommand{\U}{{\operatorname{U}}}  %unitary

%Notations - Other

\newcommand{\Ck}{{C^k}} %k-differentiable
\newcommand{\CIN}{{C^\infty}}   %infinitely differentiable
\newcommand{\ftimes}[2]{{\lrsubscripts{\times}{#1}{#2}}} %fibre product
\newcommand{\toto}{{~\rightrightarrows~}} %groupoid double arrow
\newcommand{\hook}{{\lrcorner\,}} %hook or interior multiplication
\newcommand{\limit}[1]{{\underset{#1}{\lim}}} %limit
\newcommand{\mar}{{\mathfrak{m}}}  %Marshall ideal
\newcommand{\mtrx}[2]{{\left[\begin{array}{#1}#2 \end{array}\right]}} %matrix
\newcommand{\pois}[2]{{\{#1,#2\}}}  %Poisson bracket
\newcommand{\red}[1]{{/\!/\!_{#1}\,}} %reduced space



%Hyperref Package Additions

\newcommand{\hypref}[2]{{\hyperref[#1]{#2~\ref{#1}}}}


%Work Mode commands -- Work Mode (current version modified by me) was originally sent to me by Yael Karshon, but I forget who gave it to her.

\newcommand{\ifwork}[1]{\ifthenelse{\boolean{workmode}}{#1}{}}
\newcommand{\comment}[1]{}
\newcommand{\mute}[1]{}
\newcommand{\printname}[1]{}

\ifwork{
\renewcommand{\comment}[1]{{\marginpar{*}\ \scriptsize{#1}\ }}
%\renewcommand{\mute}[1]{{\scriptsize \ #1\ }\marginpar{\scriptsize muted}}
\renewcommand{\printname}[1]
    {\smash{\makebox[0pt]{\hspace{-1.0in}\raisebox{8pt}{\tiny #1}}}}
}

\newcommand{\labell}[1] {\label{#1} \printname{#1}}


%Theorem Styles

\newcommand{\ifsection}[2]{\ifthenelse{\boolean{sections}}{#1}{#2}}

\theoremstyle{plain}
\ifsection{
    \newtheorem{theorem}{Theorem}[section]
}
{
    \newtheorem{theorem}{Theorem}
}

\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{question}[theorem]{Question}

% "End of Example" symbol

\def\eoe{\unskip\ \hglue0mm\hfill$\between$\smallskip\goodbreak} 
